Algorithmic Strategies for seizing Quantum Computing

Quantum computing is a nascent technology with prospects to have a huge impact in the world. Its current status, however, only counts on small and noisy quantum computers whose performance is limited. In this thesis, two different strategies are explored to take advantage of inherently quantum properties and propose recipes to seize quantum computing since its advent. First, the re-uploading strategy is a variational algorithm related to machine learning. It consists in introducing data several times along a computation accompanied by tunable parameters. This process permits the circuit to learn and mimic any behavior. This capability emerges naturally from the quantum properties of the circuit. Second, the unary strategy aims to reduce the density of information stored in a quantum circuit to increase its resilience against noise. This trade-off between performance and robustness brings an advantage for noisy devices, where small but meaningful quantum speed-ups can be found.

==> chapters/appendices.tex <==
%auto-ignore

\appendix

%\chapterimage{}
\chapter{Technical appendices}

\section{Classical UAT for complex functions}\label{app:real_to_complex_uat}
In this Appendix we show that the standard formulation of the UAT supports the approximation of complex function using $e^{i (\cdot)}$ as the activation function.

Let us 
follow the approximations according to the UAT of the function
\begin{equation}
    z(\vec x) = a(\vec x) + i b(\vec x), 
\end{equation}
using trigonometric functions as $\sigma(\cdot)$, 
\begin{eqnarray}
a(x) = \sum_{j=1}^N \alpha_i \cos(\vec w_j \cdot \vec x + a_j) \\
b(x) = \sum_{j=1}^N \beta_i \sin(\vec v_j \cdot \vec x + b_j).
\end{eqnarray}
Then
\begin{equation}
z(x) = \sum_{j=1}^N \alpha_i \cos(\vec w_j \cdot \vec x + a_j) + i \sum_{j=1}^N \beta_i \sin(\vec v_j \cdot \vec x + b_j),
\end{equation}

and this equation is can be rearranged as 
\begin{equation}
    z(x) = \sum_{j=1}^N \frac{\alpha_j}{2}\left( e^{i (\vec w_j \cdot \vec x + a_j)} + e^{-i ( \vec w_j \cdot \vec x + a_j)}\right) + \frac{\beta_j}{2} \left(e^{i (\vec v_j \cdot \vec x + b_j)} - e^{-i (\vec v_j \cdot \vec x + b_j)} \right),
\end{equation}

what encourages the UAT formulation for complex functions as an analogous to Eq. \eqref{eq:UAT}
\begin{equation}\label{eq:complex_UAT}
    G(\vec x) = \sum_{n=1}^N \gamma_n e^{i\delta_n} e^{i \vec u_n \cdot \vec x}.
\end{equation}


\section{Mathematical theorems for proving quantum UAT}\label{app:math_theorems}
%\begin{theorem}\label{th:hahn_banach}
%{\bf: Hahn-Banach} \cite{analysis-hahn1927, analysis-banach1929}\\
%
%Set $\mathbb{K} = \mathbb{R} {\;\rm or\;} \mathbb{C}$. Let $V$ be a $\mathbb{K}-$vector space with a seminorm $p: V \rightarrow \mathbb{R}$. If $\varphi : U \rightarrow \mathbb{K}$ is a $\mathbb{K}-$linear functional on a $\mathbb{K}-$linear subspace $U\subset V$ such that
%\begin{equation}
%|\varphi(x)| \leq p(x) \qquad \forall x \in U,
%\end{equation}
%then there exists a linear extension $\psi : V \rightarrow \mathbb{K}$ of $\varphi$ to the whole space $V$ such that
%\begin{eqnarray}
%\psi(x) = \varphi(x) \qquad \forall x\in U \\
%|\psi(x)| \leq p(x) \qquad \forall x\in V
%\end{eqnarray}
%\end{theorem}
%
%
%\begin{theorem}\label{th:riesz}
%{\bf: Riesz Representation} \cite{analysis-riesz1914}\\
%
%Let $X$ be a locally compact Hausdorff space. For any positive linear functional $\psi$ on $C(X)$, there exists a uniruq regular Borel measure $\mu$ such that
%\begin{equation}
%\forall f \in C_c(X): \qquad \psi(f) = \int_X f(x) d\mu(x)
%\end{equation}
%\end{theorem}
%
%\begin{theorem}\label{th:lebesgue}
%{\bf: Lebesgue Bounded Convergence} \cite{analysis-weir1974}\\
%Let $\lbrace f_n\rbrace$ be a sequence of complex-valued measurable functions on a measure space $(S, \Sigma, \mu)$. Suppose that $\lbrace f_n \rbrace$ converges pointwise to a function $f$ and is dominated by some integrable function $g(x)$ in the sense
%\begin{equation}
%|f_n(x)| \leq g(x), \qquad \int_S |g|d\mu < \infty
%\end{equation}
%then
%\begin{equation}
%\lim_{n\rightarrow \infty} \int_S f_n d\mu = \int_S f d\mu
%\end{equation}
%\end{theorem}

\begin{theorem}\label{th:hahn_banach}
{\bf: Hahn-Banach}\\~\cite{hahn_analysis_1927, banach_analysis_1929}\\

Set $\mathbb{K} = \mathbb{R} {\;\rm or\;} \mathbb{C}$. Let $V$ be a $\mathbb{K}-$vector space with a seminorm $p: V \rightarrow \mathbb{R}$. If $\varphi : U \rightarrow \mathbb{K}$ is a $\mathbb{K}-$linear functional on a $\mathbb{K}-$linear subspace $U\subset V$ such that
\begin{equation}
|\varphi(x)| \leq p(x) \qquad \forall x \in U,
\end{equation}
then there exists a linear extension $\psi : V \rightarrow \mathbb{K}$ of $\varphi$ to the whole space $V$ such that
\begin{eqnarray}
\psi(x) = \varphi(x) \qquad \forall x\in U \\
|\psi(x)| \leq p(x) \qquad \forall x\in V
\end{eqnarray}
\end{theorem}


\begin{theorem}\label{th:riesz}
{\bf: Riesz Representation}\\~\cite{riesz_analysis_1914}\\

Let $X$ be a locally compact Hausdorff space. For any positive linear functional $\psi$ on $C(X)$, there exists a uniruq regular Borel measure $\mu$ such that
\begin{equation}
\forall f \in C_c(X): \qquad \psi(f) = \int_X f(x) d\mu(x)
\end{equation}
\end{theorem}

\begin{theorem}\label{th:lebesgue}
{\bf: Lebesgue Bounded Convergence}\\~\cite{weir_analysis_1974}\\
Let $\lbrace f_n\rbrace$ be a sequence of complex-valued measurable functions on a measure space $(S, \Sigma, \mu)$. Suppose that $\lbrace f_n \rbrace$ converges pointwise to a function $f$ and is dominated by some integrable function $g(x)$ in the sense
\begin{equation}
|f_n(x)| \leq g(x), \qquad \int_S |g|d\mu < \infty
\end{equation}
then
\begin{equation}
\lim_{n\rightarrow \infty} \int_S f_n d\mu = \int_S f d\mu
\end{equation}
\end{theorem}

\section{Definitions of 2D functions for universality}\label{app:2D_benchmark}

\begin{figure}[b!]
\centering
    \includegraphics[width=1.2\linewidth]{model_2D.pdf}
    \caption{Graphical representation of 2-dimensional functions utilized for benchmarking. A regularization is applied to obtain $Z$ values between $-1$ and $1$ for the given domain.}
    \label{fig:2d_functions}
\end{figure}

The definitions used for the 2-dimensional functions \cite{2d_functions} that serve for benchmarking our proposed algorithms are define as

\begin{equation}
    {\rm Himmelblau}(x, y) = (x^2 + y - 11)^2 + (x + y^2 - 7)^2,
\end{equation}

\begin{equation}
{\rm Brent}(x, y) = \left(\frac{x}{2}\right)^2 + \left(\frac{y}{2}\right)^2 + e^{-\left(\left(\frac{x}{2} - 5\right)^2 + \left(\frac{y}{2} - 5\right)^2)\right)},
\end{equation}

\begin{multline}
{\rm Threehump}(x, y) = \\ = 2 \left(\frac{2 x}{5}\right)^2 - 1.05 \left(\frac{2 x}{5}\right)^4 + \frac{1}{6}\left(\frac{2 x}{5}\right)^6 + \\ + \left(\frac{2 x}{5}\right) \left(\frac{2 y}{5}\right) + \left(\frac{2 y}{5}\right)^2,
\end{multline}

\begin{equation}
{\rm Adjiman}(x, y) = \cos(x) \sin(y) - \frac{x}{y^2 + 1},
\end{equation}

where a normalization to $-1 \leq f(x, y) \leq 1$ is applied after this definition. A graphical representation of these functions is depicted in Fig. \ref{fig:2d_functions}.

\section{Superconducting experiment for a universal approximant}\label{app:exp_universal}

The experimental implementation of the single-qubit universal approximant as detailed in Sec.~\ref{sec:benchmark} was performed in a superconducting qubit circui. The qubit is a 3D transmon geometry~\cite{3d-transmon} located inside an aluminum three-dimensional cavity. The cavity bare frequency, $\omega_c = 2\pi \times 7.89$ GHz, is greatly detuned from the qubit frequency, $\omega_q = 2\pi \times 4.81 $ GHz. Hence, there is a qubit state-dependent dispersive shift on the cavity resonance, $2\vert\chi\vert = 2\pi \times 1.5 $MHz. The qubit anharmonicity is $\alpha = -2\pi \times 324$ MHz and the qubit relaxation and spin-echo decay times are, respectively, $T_1 = 15.6~\mu s$ and $T_{2Echo} = 12.0~\mu s$. These time scales exceed the operation times needed to implement the algorithm up to 6 layers by 2 orders of magnitude. See Fig.~\ref{fig:coh-times} for a experimental fit on these times. 

\begin{figure}
\includegraphics[width=.8\linewidth]{Coherence_times.pdf}

\caption{$T_1$ measurement with exponential fit (top) and spin-echo measurement, $T_{2E}$, with exponential fit (bottom).}
\label{fig:coh-times} 
\end{figure}

The experiment was realized in a dilution fridge with a base temperature of approximately $20$~mK. The qubit rotation pulses were defined by an arbitrary waveform generator (AWG) and then upconverted with a microwave signal generator to the gigahertz frequency range before being sent to the qubit/cavity system. The signal was low-pass filtered and attenuated by a total of 50dB before reaching the aluminum cavity. The input port of the cavity was undercoupled while the output port was overcoupled in order to maximize the readout signal amplitude. The outgoing signal was amplified by a cryogenic low noise amplifier and a second amplification stage at room temperature. The downconversion is performed with the same microwave generator as used in the upconversion of the measurement pulse, guaranteeing phase coherence in the downconversion process. The signal is read out in a digitizer, with a FPGA that demodulates and averages the results before sending the data to the main measurement computer.

\begin{figure}
\centering
\subfigure[\hspace{2mm} Full sequence]{\includegraphics[width=.45\linewidth]{Full_Sequence.png}} \hfill 
\subfigure[\hspace{2mm} Pulse sequence]{\includegraphics[width=.45\linewidth]{Pulse_sequence.png}}
\caption{a) Complete pulse sequence. First, the reset protocol is performed which corresponds to two pulses at the cavity and the qubit frequencies, respectively. Note that the qubit pulse is of considerably lower amplitude than the cavity pulse. Also, both pulses have a longer duration than the qubit rotation sequence (timings not to scale). The ``Y" pulses are shown to have different amplitudes to determine each rotation angle. Finally, the readout corresponds to a pulse at the cavity frequency which is later read out by a digitizing card. b) Sequence performed in the experiment. Blue boxes represent actual pulses. Logical Y and Z rotations are explicitly shown below the blue boxes~\cite{virtual-zgates}. Note that Z pulses do not correspond to any microwave pulse, instead subsequent pulses change rotation axis, indicated by a prime, $Y_N^{(N)}$.}
\label{fig:exp_gates} 
\end{figure}

In order to implement the gate sequences defined in the previous section we follow the correspondence between logical and physical gates as shown in Fig.~\ref{fig:exp_gates}. The phase of each pulse is selected at the pulse generator to modify the rotation axis, producing either X or Y rotations as required. The Z rotations are, in turn, virtual~\cite{virtual-zgates}. The microwave pulses incorporate a DRAG correction~\cite{drag-a,drag-b} which leads to an error per gate $\epsilon = 0.01$ found with randomized benchmarking~\cite{randomized-benchmarking}, see Fig.~\ref{fig:drag}. Randomized benchmarking measures errors in Clifford gates and not arbitrary angle rotations, which are instead used in this experiment, yet offers a reasonable estimate on the overall fidelity of our gates. The gate error observed is probably limited due to a non-ideal filtering of the measurement lines in the fridge. In order to achieve better qubit state readout visibility and shorter operation times, a reset protocol is applied prior to the main sequence \cite{reset-protocol}. 

\begin{table}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ *{13}{l} }
      \toprule
      \multicolumn{1}{c}{\textbf{Optimal}} 
      & \multicolumn{1}{c}{$p_1$}  & \multicolumn{1}{c}{$p_2$}  & \multicolumn{1}{c}{$p_3$}
      & \multicolumn{1}{c}{$p_4$}  & \multicolumn{1}{c}{$p_5$}  & \multicolumn{1}{c}{$p_6$}
      & \multicolumn{1}{c}{$p_7$}  & \multicolumn{1}{c}{$p_8$}  & \multicolumn{1}{c}{$p_9$}
      & \multicolumn{1}{c}{$p_{10}$}  & \multicolumn{1}{c}{$p_{11}$}  & \multicolumn{1}{c}{$p_{12}$}
      \\
      \textbf{parameters}
      & -2.501 & 1.685 &   1.757 & 2.105 & 3.822 & -1.788 &
 -1.507 & -4.640 & 0.430 & 1.875 & 5.038 & -1.906
      \\[0.2cm]
      \hline
      \multicolumn{1}{c}{\textbf{Rotational}} 
      & \multicolumn{2}{c}{$Z_1$}   & \multicolumn{1}{c}{$Y_1$}
      & \multicolumn{2}{c}{$Z_2$}   & \multicolumn{1}{c}{$Y_2$}
      & \multicolumn{2}{c}{$Z_3$}   & \multicolumn{1}{c}{$Y_3$}
      & \multicolumn{2}{c}{$Z_4$}   & \multicolumn{1}{c}{$Y_4$}
      \\
      \multicolumn{1}{c}{\textbf{angles$^*$}} 
      & \multicolumn{2}{c}{$p_1  + p_2 x$}   & \multicolumn{1}{c}{$p_3$}
      & \multicolumn{2}{c}{$p_4 + p_5 x$}   & \multicolumn{1}{c}{$p_6$}
      & \multicolumn{2}{c}{$p_7 + p_8 x$}   & \multicolumn{1}{c}{$p_3$}
      & \multicolumn{2}{c}{$p_{10} + p_{11} x$}   & \multicolumn{1}{c}{$p_{12}$}
      \\[0.2cm]
      \multicolumn{1}{c}{\textbf{$x=-0.5$}} 
      & \multicolumn{2}{c}{2.939}
& \multicolumn{1}{c}{1.757}
& \multicolumn{2}{c}{0.194}
& \multicolumn{1}{c}{4.495}
& \multicolumn{2}{c}{0.813}
& \multicolumn{1}{c}{0.430}
& \multicolumn{2}{c}{5.639}
& \multicolumn{1}{c}{4.377}
      \\
      \multicolumn{1}{c}{\textbf{$x=0$}} 
      & \multicolumn{2}{c}{3.782}
& \multicolumn{1}{c}{1.757}
& \multicolumn{2}{c}{2.105}
& \multicolumn{1}{c}{4.495}
& \multicolumn{2}{c}{4.776}
& \multicolumn{1}{c}{0.430}
& \multicolumn{2}{c}{1.875}
& \multicolumn{1}{c}{4.377}
      \\
      \multicolumn{1}{c}{\textbf{$x=1$}} 
      & \multicolumn{2}{c}{5.467}
& \multicolumn{1}{c}{1.757}
& \multicolumn{2}{c}{5.927}
& \multicolumn{1}{c}{4.495}
& \multicolumn{2}{c}{0.136}
& \multicolumn{1}{c}{0.430}
& \multicolumn{2}{c}{0.630}
& \multicolumn{1}{c}{4.377}
      \\[0.2cm]
      \hline
      \multicolumn{9}{l}{\small  $^*$ Angles between $0$ and $2\pi$}        
    \end{tabular}}
    \caption{Optimal parameters and angles obtained for $\relu(x)$ and 4 layers. Above the 12 parameters that define the rotational angles obtained through simulations. Below the corresponding angles of the 8 rotations for three different values of $x$. Note that Y rotations are not $x$-dependent, hence they are equal for all three $x$ values.}
    \label{tab:rotation angles}
    
\end{table}

\begin{figure}[b!]
\centering
\includegraphics[width=.7\linewidth]{DRAG.pdf}
\caption[Randomized Benchmarking]{Randomized benchmarking of the DRAG corrected pulses. The fit corresponds to the expression $Ap^n + B$, where $A$ and $B$ have dimensions of voltage, $n$ is the number of Clifford gates, and $p$ is the fidelity per gate. $\epsilon = 1-p$ is the error per gate.}
\label{fig:drag} 
\end{figure}

Figure~\ref{fig:exp_gates} shows the total pulse sequence, which includes preparation and measurement pulses in addition to the pulse sequence shown in the main text. The Y rotations are performed through microwave pulses at the qubit frequency while the Z rotations, as already stated, are phase changes in subsequent pulses. Both qubit and cavity pulses are generated at $70$~MHz and then upconverted to the gigahertz range. The qubit pulses are Gaussian pulses with a total duration of $21$~ns. A proper DRAG correction is performed with a resulting error per gate of $\epsilon = 0.01$ as shown in Fig.~\ref{fig:drag}. The cavity pulse has a total length of around $2~\mu$s. The reset protocol consists of a pulse driving the qubit and a pulse driving the cavity mode, with a total duration of around $2~\mu$s. An example of the rotation angles for the $\relu(x)$ function in the 4-layer case is shown in Table~\ref{tab:rotation angles}. 

The readout consists of a cavity tone at the frequency of the cavity for the qubit in the $\ket{0}$ state. High/low transmission corresponds to the qubit being in the ground/excited state, assuming the system does not escape from the computational basis. Each data point requires around $50000$ measurements in order to average out the amplifier noise. A reset protocol that drives the qubit into the ground state is implemented prior to each individual sequence. This has two benefits. The first one allows us to start with a qubit state nearly polarized into the ground state. A second benefit is the reduction in the overall duration of the experiment, since the waiting time between individual measurements is not limited by the qubit relaxation time.

\section{Appendix for ion trap}


\section{Quantum circuits in NNPDF methodology}\label{app:nnpdf}

The latest implementation of the latest iteration of the NNPDF methodology is described in Ref.~\cite{Carrazza:2019mzf}.
This implementation is very modular and one can seamlessly swap the \texttt{Tensorflow} based backend by any other
provider.
{\tt Qibo}, which is also partially based on \texttt{Tensorflow} can be easily integrated with the NNPDF methodology.

As previously mentioned, all results in this section corresponds to the simulation of the quantum device on classical hardware.
Such a simulation is very costly from a computational point of view which introduces a number of limitations
that need to be addressed in order to produce results in reasonable time frames.

{\bf FK reduction}: the definition of the quantum circuit depends on both the set of parameters $\theta$ and the value of
the parton momentum fraction $x$ (see Eq.~\eqref{eq:quantumcircuit}) which means the circuits needs to be simulated
once per value of $x$.
The union of all FK tables for all physical observables (following Eq.~\eqref{eq:convolution}) amounts to
several thousand values of $x$.
Since such a large number of evaluations of the quantum circuit is impracticable, we introduce a further approximation
where each partial FK table is mapped to a fixed set of 200 nodes in the x-grid.
This simplification introduces an error to the total $\chi^{2}$ of the order of $\Delta\chi^{2} = 0.14 \pm 0.01 $ when averaged
over PDF members.
This error on the cost function is however negligible for the accuracy reached in this work.

{\bf Positivity}: in the fitting basis, as defined in section~\ref{ssec:qcpdf}, the PDF cannot go negative.
Physical predictions however are computed in the flavour basis~\cite{Ball:2008by} where the rotation between basis
can make some results go negative.
However, physical observables (differential or total cross sections) cannot be. This physical constraint is included in NNPDF3.1 via fake pathological datasets.
These have not been implemented for qPDF as they correspond to a fine-tuning of the methodology which is beyond the
scope of this work.

The removal of the positivity constraint from the fit introduces an unphysical distortion to the results as the PDF
could produce negative predictions for physical predictions. Such results are unphysical because they would correspond
to situations in which the probability of finding a particular phase space configuration is negative, which makes no
sense.
In Fig.~\ref{fig:positivity} we compare the ``negativity'' between qPDF and a version of NNPDF3.1 with the positivity constraints removed.
We observe that both fits behave similarly, proving such unphysical results are a consequence of the removal of the
constraint rather than a problem in the qPDF methodology.

{\bf Momentum Sum Rule}: the PDFs as defined in Eq.~\eqref{eq:nnpdf} are normalized such that~\cite{Ball:2014uwa},
\begin{equation}
    \frac{\displaystyle\int_0^1 dx \; x\,f_{g}(x,Q_0)}{1-\displaystyle\int_0^1 dx  x f_{\Sigma}(x,Q_0)} \simeq 1,
\end{equation}
this equation is known as the momentum sum rule and it is imposed in \texttt{n3fit}
through an integration over the whole range of x which is impracticable
% \begin{align}
%     \frac{\displaystyle\int_0^1 dx \; x\,f_{g}(x,Q_0)}{1-\displaystyle\int_0^1 dx  x f_{\Sigma}(x,Q_0)} &\simeq 1;
%         \quad \displaystyle\int_0^1 dx \, f_{V}(x,Q_0) &\simeq 3; \nonumber\\
%     \displaystyle\int_0^1 dx \, f_{V_3}(x,Q_0) &\simeq 1;
%         \quad \displaystyle\int_0^1 dx \, f_{V_8}(x,Q_0) &\simeq 3;\nonumber
% \end{align}
% these rules are imposed in \texttt{n3fit} through an integration over the whole range of x which is impracticable
in this implementation for the reasons mentioned above.
Instead, in qPDF these are only checked afterwards, finding a good agreement with the expected values (despite not being
imposed at fitting time).
Indeed, for qPDF the result for the average over all replicas is $ 1.01\pm 0.01$, 
which is to be compared with the NNPDF3.1 result of $1.000 \pm 0.001$, where the constraint was imposed at fit time.

\subsubsection{Extra results}
With all ingredients implemented, we are in a position to run a NNPDF3.1-like fit using the qPDF.
As a base reference for the comparison we take the NNPDF3.1 NNLO fit~\cite{Ball:2017nwa},
which is the latest release by the NNPDF collaboration.
The plots comparing the NNPDF sets with qPDF are then produced using a
\texttt{reportengine}~\cite{zahari_kassabov_2019_2571601} based internal NNPDF tool. The extra result here presented complement the one showed in the main text, in particular related to Fig.~\ref{fig:fitperflavour}. 

\begin{figure}[h!]
\begin{adjustwidth}{-2cm}{-1cm}
\begin{minipage}{.47\linewidth}
\subfigure[$\chi^{2}/N$ per experiment grouping. There is a deterioration of the goodness of the
        fit (measured by the $\chi^{2}$) for some of the experiments for the central value.
        The goodness of the fit is very similar between the reference and
        qPDF for most of the experiments being considered.\label{fig:expchi2}]{\includegraphics[width=\linewidth]{exp_chi2.pdf}}
\end{minipage}
\hfill
\begin{minipage}{.47\linewidth}
\subfigure[Predictions for a toy $s\bar{s}$ initiated Drell-Yan process with qPDF and a simplified version of NNPDF3.1
    where the positivity constraint has been removed.\label{fig:positivity}]{\includegraphics[width=\linewidth]{positivity.pdf}} 
\subfigure[Distance (as defined by Eq.~\eqref{eq:distance}) between qPDF and NNPDF3.1. When the distance is kept
    under $d(f_{i}, r_{i})=10$ the two fits are 1-$\sigma$ compatible. All partons except for $u$ and $s$ are below or
    around the 1-$\sigma$ distance for the entire range considered. Note however, by comparing to
Fig.~\ref{fig:all_flavours} that the fits for both the $u$ and $s$ quarks are compatible in the most relevant regions
for these particles.\label{fig:distance}]{\includegraphics[width=\linewidth]{distances.pdf}}
\end{minipage}
\end{adjustwidth}
\caption{Collection of extra results for the qPDF method integrated in the NNPDF methodology as extracted from LHC data. }
\end{figure}

We can start by comparing the $\chi^{2}/N$ result for the datasets that have been considered in the fit,
shown in Fig.~\ref{fig:expchi2}.
One would expect a perfect fit when $\chi^{2}/N = 1$,
however this is not the case even in the reference and it is due to a combination of missing higher order corrections
(a lack of a better theory) or inconsistencies in the experimental results.
The similarity on the phenomenological results obtained by both fitting methodologies as shown in Fig.~\ref{fig:expchi2}
is well understood as well by looking at the distance plots between the qPDF~and the reference in
Fig.~\ref{fig:distance},
\begin{equation}
    d^2(f_{i}, r_{i}) = \frac{\langle f_{i} \rangle - \langle r_{i} \rangle}{\frac{1}{N_f}\sigma(f_{i})^2 +
    \frac{1}{N_{r}}\sigma(r_{i})^2},\label{eq:distance}
\end{equation}
where $i$ is the flavour being considered and $f$ and $r$ corresponds to qPDF~and the reference (NNPDF3.1)
respectively. The central value is taken over the $N$ replicas of the set, generally of the order of 100.

\begin{figure}[t!]
    \centering
\begin{adjustwidth}{-1cm}{-2cm}
    \subfigure[\ Atlas jets data differential in rapidity~\cite{Aad:2014vwa}.]{
        \includegraphics[width=0.31\linewidth]{atlasexp.pdf}
    } \hfill
    \subfigure[\ CMS Z differential in rapidity for fixed value of $p_{T}$~\cite{Khachatryan:2015oaa}.]{
        \includegraphics[width=0.31\linewidth]{cmsexp.pdf}
    } \hfill
    \subfigure[\ LHCb, Z cross section differential in rapidity~\cite{Aaij:2012vn}.]{
        \includegraphics[width=0.31\linewidth]{lhcbexp.pdf}
    }
    \end{adjustwidth}
    \caption{Theoretical predictions computed with the method describe in~\cite{Bertone:2016lga} in order to compare
    the same prediction with three different PDF sets. We note that the predictions for the qPDF set is compatible with
both the experimental measurements and the released PDF set. The parton-level calculation has been performed with the
NLOjet++~\cite{Nagy:2001fj} and MCFM~\cite{Campbell:2019dru} tools.}\label{fig:expresults}
\end{figure}

Indeed, for most partons the difference between both fits are under the 1-$\sigma$ level (distance equal to 10 for 100
replicas) growing up to 2-$\sigma$ for the $u$ and $s$ quarks.

\begin{figure}[b!]
  \includegraphics[width=\linewidth]{correlations.pdf}
  \caption{\label{fig:correlation}PDF correlation matrix for flavours in a grid
  of $x$ points for NNPDF3.1 NNLO (left) and the qPDF (right).}
\end{figure}

%This point is clearly seen in Fig.~\ref{fig:fitperflavour} where we compare the
%published PDFs (with their corresponding error bars) for the gluon and the $d$ and
%$u$ quarks. We note that for these quark flavours the qPDF central result is almost
%always within the 1-$\sigma$ range of the reference, with an overlapping error
%band for the whole considered range.

In Fig.~\ref{fig:expresults} we show specifically a comparison between the reference NNPDF3.1 and qPDF for selected
datasets, we also provide the LHAPDF-compatible PDF grid.
We observe that the accuracy of the qPDF central value is similar to that of NNPDF3.1.
Furthermore, the error bars for the predictions of both PDF set overlap with the experimental error bars, and, in some
cases, also among themselves.

Finally, in Fig.~\ref{fig:correlation} we compute the PDF correlations for
NNPDF3.1 and qPDF replicas using Pearson's coefficient in a fixed grid of 100
points distributed logarithmically in $x=[10^{-4},1]$.

This leads us to conclude that the methodology described in this paper can be used for regression problems to unknown functional
forms such as the proton internal structure and produce results that are perfectly coherent, from a phenomenological
point of view, with the state of the art.
In addition we believe that with adequate tuning one could achieve the same level of accuracy of the classical
approach.

We finalize this section by showing phenomenological results where the LHAPDF grids produced with this approach are used
for a full fixed order prediction.
In summary going back circle to the master equation, i.e., computing numerically Eq.~\eqref{eq:convolution}
with no approximations using state of the art tools.

